PARIS and ELSA: An Elastic Scheduling Algorithm for Reconfigurable Multi-GPU Inference Servers

In cloud machine learning (ML) inference systems, providing low latency to end-users is of utmost importance. However, maximizing server utilization and system throughput is also crucial for ML service providers as it helps lower the total-cost-of-ownership. GPUs have oftentimes been criticized for ML inference usages as its massive compute and memory throughput is hard to be fully utilized under low-batch inference scenarios. To address such limitation, NVIDIA's recently announced Ampere GPU architecture provides features to "reconfigure" one large, monolithic GPU into multiple smaller "GPU partitions". Such feature provides cloud ML service providers the ability to utilize the reconfigurable GPU not only for large-batch training but also for small-batch inference with the potential to achieve high resource utilization. In this paper, we study this emerging GPU architecture with reconfigurability to develop a high-performance multi-GPU ML inference server. Our first proposition is a sophisticated partitioning algorithm for reconfigurable GPUs that systematically determines a heterogeneous set of multi-granular GPU partitions, best suited for the inference server's deployment. Furthermore, we co-design an elastic scheduling algorithm tailored for our heterogeneously partitioned GPU server which effectively balances low latency and high GPU utilization.

==> tex/discussion.tex <==
\section{Related Work}
\label{sect:discussion}

Because of the rapidly increasing complexity of DNN-based ML algorithms, the
computer architecture community has witnessed a surge of interest in ML
accelerator architectures with a strong emphasis on accelerating CNNs, RNNs, and
MLPs~\cite{diannao,dadiannao,shidiannao,pudiannao,du:2015:micro,minerva,dnn_pim_reram,eyeriss,cambricon,isacc,neurocube,redeye,tabla,dnnweaver,intel:2017:fpl,gao:2017:tetris,intel:2018:fpga,rhu:2016:vdnn,song:2015:eie,cnvlutin,cambriconx,stripes,bitpragmatic,intel:2017:icassp,intel:2017:fpga,whatmough:2017:isscc,whatmough:2017:hotchips,scnn,bittactical,rhu:2018:cdma,tpu1}.
As the focus of these prior work is on designing a single NPU in isolation, little
attention has been paid in \emph{how} the ML inference server collects the batched
inputs to feed it into these NPU architectures. The key objective of our \lazyb
design is to study the implication of batching on the system-level latency,
			 throughput, and QoS which is a rare contribution in our community given
			 its primary focus on ML accelerator design so far.  In general, the
			 contributions and intuitions behind our proposed \lazyb architecture can
			 readily be applied to prior NPU proposals and is hence orthogonal to the
			 closely related prior work above.


